A Graph-Based Technique for the Automated Control-Oriented Modeling of District Heating Networks

Advanced control strategies for delivering heat to users in a district heating network have the potential to improve performance and reduce wasted energy. To enable the design of such controllers, this paper proposes an automated plant modeling framework that captures the relevant system dynamics, while being adaptable to any network configuration. Starting from the network topology and system parameters, the developed algorithm generates a state-space model of the system, relying on a graph-based technique to facilitate the combination of component models into a full network model. The accuracy of the approach is validated against experimental data collected from a laboratory-scale district heating network. The verification shows an average normalized root mean square error of 0.39 in the mass flow rates delivered to the buildings, and 0.15 in the network return temperature. Furthermore, the ability of the proposed modeling technique to rapidly generate models characterizing different network configurations is demonstrated through its application to topology optimization. The optimal design, obtained via a branch and bound algorithm, reduces network heat losses by 15% as compared to the conventional length-minimized topology.

==> scrap.tex <==
\begin{enumerate}
    \item $A_{11}\in\mathbb{R}^{n_s\times n_s}$ represents the connections of split nodes to the feeding network. In the example, it would contain a term for $v_7$.
    \item $A_{12}\in\mathbb{R}^{n_s\times n_p}$ represents the connection of the feeding lines of users to split nodes. In the example, it would contain a term to connect $v_3$ to $v_7$.
    \item $A_{21}\in\mathbb{R}^{n_p\times n_s}$ represents the connection of the feeding lines of split nodes to users. In the example, it would contain terms to connect $v_7$ to $\{v_4, v_5\}$.
    \item $A_{22}\in\mathbb{R}^{n_p\times n_p}$ represents the dynamics within users and between the users feeding and return lines. In the example, it would contain six block diagonal elements for $\{v_1 \dots v_6\}$, above-the-diagonal block elements for $\{v_1, v_2,v_5\}$ and below-the-diagonal block elements for $\{v_2,v_3,v_6\}$.
    \item $A_{23}\in\mathbb{R}^{n_p\times n_s}$ represents the connection of the return line of split nodes to users. In the example, it would contain a term to connect $v_7$ to $v_3$.
    \item $A_{32}\in\mathbb{R}^{n_s\times n_p}$ represents the connection between of return lines in users to split nodes. In the example, it would contain terms to connect $\{v_4,v_5\}$ to $v_7$.
    \item $A_{33}\in\mathbb{R}^{n_s\times n_s}$ represents the connections of split nodes to the feeding network. In the example, it would contain a term for $v_7$.\
\end{enumerate}

 The network shown in \cref{fig:ex} was converted to its graph representation, depicted in \cref{fig:exgraph}, and will be used as a case study for the complete modeling method. The characteristics of this sample network are summarized in \cref{table:ex}.

\begin{figure}
    \centering
    \includegraphics[width = 2in]{fig/examplegraph.eps}
    \caption{Topology graph of sample six user DHN.}
    \label{fig:exgraph}
\end{figure}
\begin{table}
\caption{Network size parameters for the sample network.}
\label{table:ex}
\centering
\begin{tabular}{l c c}
\toprule
Parameter & Symbol & Value\\
\midrule
\# of Users & $n_u$ & 6\\
\# of Split Nodes & $n_s$ & 1\\
\# of Loop Segments & $n_p$ & 32\\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
A model of the economic cost of installation and impact of the graph configuration on fluid flow has been developed to minimize the upfront installation installation cost of a new network based on the chosen pipe diameter \cite{wackEconomicTopologyOptimization2023}. Finally, a modified genetic algorithm has been used to design the optimal graph layout to minimize installation costs and pressure drops in a new DHN configuration \cite{suOptimizingPipeNetwork2022}. While a variety of graph based models exist, none have been used for generating dynamic models of a DHN.\par 
\end{comment}

\begin{comment}
Additionally, a vast majority of physics-based DHN models are implemented within a specific simulation software framework. For example, a Simulink library has been developed, with blocks for the buildings, heat sources, and network components \cite{gambarottaLibrarySimulationSmart2017}. Modelica is also commonly used in the implementation of different modeling techniques, and many DHN specific libraries have been developed including the INDIGO project \cite{delhoyoarceModelsFastModelling2018}, OPTi-Sim \cite{simonssonExperiencesCityScaleSimulation2021}, and CityGML  \cite{husseinModellingValidationDistrict2021}. However, very few models allow for a more generalized implementation.\par
A more generalizable, matrix-based approaches have been used for calculating the mass flow rate in water distribution networks \cite{todiniUnifiedFrameworkDeriving2013}. They have also been used in calculating the steady state temperature behavior of a DHN \cite{wangMethodSteadystateThermal2016}, but have not been used for the development of a dynamic model of a large-scale DHN.\par
\end{comment}

\begin{table*}[t]
\caption{Calibrated $h$ values ($[W/K]$).}
\label{tble:h}
\centering
\begin{tabular}{cccccccccccccccc}
\toprule
$\{3\}$&$\{1\}$&$\{1\}$&$\{1\}$&$\{1\}$&$\{1\}$&$\{1\}$&$\{2\}$&$\{2\}$&$\{2\}$&$\{2\}$&$\{2\}$&$\{2\}$&$\{3\}$\\
F&F&S1&S2&S3&R&B&F&S1&S2&S3&R&B&R\\
\midrule
3.759&
0.0102&301.1&$1.627\times10^3$&0.0163&0.0134&0.0036&
0.0040&244.0&$1.408\times10^3$&0.0126&0.0121&0.0036&
0.0016\\
\bottomrule
\end{tabular}
\end{table*}
